The Kernel Interaction Trick: Fast Bayesian Discovery of Pairwise Interactions in High Dimensions

Discovering interaction effects on a response of interest is a fundamental problem faced in biology, medicine, economics, and many other scientific disciplines. In theory, Bayesian methods for discovering pairwise interactions enjoy many benefits such as coherent uncertainty quantification, the ability to incorporate background knowledge, and desirable shrinkage properties. In practice, however, Bayesian methods are often computationally intractable for even moderate-dimensional problems. Our key insight is that many hierarchical models of practical interest admit a particular Gaussian process (GP) representation; the GP allows us to capture the posterior with a vector of O(p) kernel hyper-parameters rather than O(p^2) interactions and main effects. With the implicit representation, we can run Markov chain Monte Carlo (MCMC) over model hyper-parameters in time and memory linear in p per iteration. We focus on sparsity-inducing models and show on datasets with a variety of covariate behaviors that our method: (1) reduces runtime by orders of magnitude over naive applications of MCMC, (2) provides lower Type I and Type II error relative to state-of-the-art LASSO-based approaches, and (3) offers improved computational scaling in high dimensions relative to existing Bayesian and LASSO-based approaches.

==> boston.tex <==
%
\begin{table}[h]
\caption{Boston housing dataset results. RMSE denotes the out-of-sample root-mean squared error for the predictions. The last two columns indicate the number of main effects and pairwise effects selected by each method.}
\label{table:boston_data}
\begin{center}
\begin{small}
\begin{sc}
\begin{tabular}{lcccr}
\toprule
Method & RMSE & \# Main &  \# Pairwise \\ 
\midrule
SKIM    & 3.95 & 3 & 0 \\
PLASSO & 3.88 & 9& 42\\
HLASSO    & 4.07 & 12& 24 \\
\bottomrule
\end{tabular}
\end{sc}
\end{small}
\end{center}
\end{table}
%

==> mult_kern_int_trick.tex <==
Without any loss of generality, we show how to recover the joint posterior distribution of any set of parameters $\theta_{i_k}$, $1 \leq k \leq K \leq p$, and their pairwise interactions $\theta_{i_k i_s}$ for $s \leq K$. Let
\begin{equation}
A^{KK} \coloneqq [e_{i_1} -e_{i_1} \cdots e_{i_K} -e_{i_K} e_{i_1 i_2} \cdots e_{i_{K-1} i_K} ]^T.
\end{equation}
Following the proof of \cref{prop:formula_marginal},
\begin{equation} \label{eq:mult_joint_dist}
\begin{split}
& g(A^{KK}) \mid D, \tau \sim N(\mu_{g_{KK}}, \Sigma_{KK}) \quad \text{s.t.} \quad \mu_{g_{KK}} \coloneqq  K_{\tau}(A^{KK}, X) H_{\tau} Y, \\
	& \qquad \Sigma_{KK} \coloneqq  \left[K_{\tau}(A^{KK}, A^{KK}) - K_{\tau}(A^{KK}, X) H_{\tau} K_{\tau}(X, A^{KK})  \right]. 
\end{split}
\end{equation}
Now, the joint posterior distribution of these parameters can be obtained from  \cref{eq:mult_joint_dist} using nearly an identical procedure as in \cref{eq:test_point_select}.
